A Logic-based Multi-agent System for Ethical Monitoring and Evaluation of Dialogues

Dialogue Systems are tools designed for various practical purposes concerning human-machine interaction. These systems should be built on ethical foundations because their behavior may heavily influence a user (think especially about children). The primary objective of this paper is to present the architecture and prototype implementation of a Multi Agent System (MAS) designed for ethical monitoring and evaluation of a dialogue system. A prototype application, for monitoring and evaluation of chatting agents' (human/artificial) ethical behavior in an online customer service chat point w.r.t their institution/company's codes of ethics and conduct, is developed and presented. Future work and open issues with this research are discussed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{182}
\providecommand{\publicationstatus}{A. Formisano, Y.A Liu, et al. (Eds.): International Conference on\\ Logic Programming (Technical Communications) 2021 (ICLP 2021)\\
EPTCS 345, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.345.32}{10.4204/EPTCS.345.32}}
\pdfoutput=1

